Hybrid Collaborative Filtering Models for Clinical Search Recommendation

With increasing and extensive use of electronic health records, clinicians are often under time pressure when they need to retrieve important information efficiently among large amounts of patients' health records in clinics. While a search function can be a useful alternative to browsing through a patient's record, it is cumbersome for clinicians to search repeatedly for the same or similar information on similar patients. Under such circumstances, there is a critical need to build effective recommender systems that can generate accurate search term recommendations for clinicians. In this manuscript, we developed a hybrid collaborative filtering model using patients' encounter and search term information to recommend the next search terms for clinicians to retrieve important information fast in clinics. For each patient, the model will recommend terms that either have high co-occurrence frequencies with his/her most recent ICD codes or are highly relevant to the most recent search terms on this patient. We have conducted comprehensive experiments to evaluate the proposed model, and the experimental results demonstrate that our model can outperform all the state-of-the-art baseline methods for top-N search term recommendation on different datasets.

==> tables/cutoff.tex <==
\begin{table}[h]
\small
  \caption{Dataset Statistics based Cut-off Time}
  \centering
  \vspace{-8pt}
  \label{tbl:dataset}
  \begin{threeparttable}
      %\begin{footnotesize}
      \begin{tabular}{
        @{\hspace{0pt}}l@{\hspace{8pt}}
        @{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
	@{\hspace{8pt}}r@{\hspace{8pt}}
        }
        \toprule
        Cut-off Time & \#Pr$_{tr}$ & \#Pr$_{te}$ & \#Tr$_{tr}$ & \#Tr$_{te}$ \\
        \midrule
        Apr. 1st 2015 &  2,854 & 109 & 1,915 & 442 \\
        Oct. 1st 2014 &  2,224 & 20  & 1,493 & 56  \\
        Apr. 1st 2014 &  1,171 & 139 & 1,065 & 254 \\
        Oct. 1st 2013 &  249   & 11  & 373   & 32  \\

        \bottomrule
      \end{tabular}
      %\end{footnotesize}

    %  \begin{tablenotes}[normal,flushleft]
    %  \begin{scriptsize}
      
    %  \end{scriptsize}
    %  \end{tablenotes}
  \end{threeparttable}
  \vspace{-15pt}
\end{table}


==> tables/results.tex <==

\begin{table*}[ht!]
\small
  \caption{Performance Comparison for All Methods with Cut-off Time April 1st, 2015}
  \centering
  \label{tbl:results20150401}
  \begin{threeparttable}
      \begin{tabular}{
	@{\hspace{6pt}}l@{\hspace{6pt}}
        @{\hspace{0pt}}r@{\hspace{6pt}}
	@{\hspace{0pt}}r@{\hspace{6pt}}
        @{\hspace{0pt}}r@{\hspace{0pt}}
	@{\hspace{0pt}}l@{\hspace{6pt}}
	@{\hspace{0pt}}r@{\hspace{6pt}}          
	@{\hspace{6pt}}r@{\hspace{6pt}}
	@{\hspace{6pt}}r@{\hspace{6pt}}
	@{\hspace{6pt}}r@{\hspace{6pt}}
        @{\hspace{6pt}}r@{\hspace{6pt}}
        @{\hspace{6pt}}r@{\hspace{6pt}}
        @{\hspace{6pt}}r@{\hspace{6pt}}
        %@{\hspace{6pt}}r@{\hspace{6pt}}
	}
        \toprule
        method      & \multicolumn{3}{r}{parameters}  &  & HR@1  & HR@2 & HR@3 & HR@4 & HR@5 & HR@10 & HR@20 \\ %& HR@40 \\

        \midrule
\multirow{2}{*}{\baseline}  &   $s_p$ & $s_t$ & $\alpha$ & & \multirow{2}{*}{\underline{0.0859}} & \multirow{2}{*}{\underline{0.1309}} & \multirow{2}{*}{0.1595} & \multirow{2}{*}{0.1861} & \multirow{2}{*}{0.2045} & \multirow{2}{*}{0.2638} & \multirow{2}{*}{0.3722} \\ %& 0.4151 \\
\cline{2-4}
           &   $0.1$ & $0.1$ & $0.9$ & & & & & & & &\\
\personlized                  & & & & & 0.0734 & 0.1193 & \underline{0.1835} & \underline{0.2110} & \underline{0.2294} & 0.2844 & 0.3211 \\ % & 0.3486 \\
\encounter                       & & & & & 0.0642 & 0.1284 & \underline{0.1835} & \underline{0.2110} & 0.2202 & \underline{0.3303} & \underline{0.4128} \\ %& 0.4862 \\
\multirow{2}{*}{\HGN} & $n_h$ & $n_p$ & & &    \multirow{2}{*}{0.0654} &  \multirow{2}{*}{0.1002} &  \multirow{2}{*}{0.1309} &  \multirow{2}{*}{0.1391} &  \multirow{2}{*}{0.1616} &  \multirow{2}{*}{0.2188} &  \multirow{2}{*}{0.3395}  \\ 
\cline{2-3}
& $20$ & $3$  & & & & & & & & &\\
\multirow{2}{*}{\HAM} & $ n_h$ & $n_l$ & $n_p$ && \multirow{2}{*}{0.0675} &  \multirow{2}{*}{0.0941} &  \multirow{2}{*}{0.1145} &  \multirow{2}{*}{0.1391} &  \multirow{2}{*}{0.1616} &  \multirow{2}{*}{0.1943} & \multirow{2}{*}{0.3211}  \\ 
\cline{2-4}
& $9$ & $1$  & $2$  & & & & & & & &\\
        \midrule

	& $m_s$ & $m_c$  & $\alpha$ & & & & & & & &\\
\cline{2-4}
\logmean (best HR@1)&  3  & 1 & 1.0  && \textbf{0.0917} & 0.1284 & 0.1743 & 0.2202 & 0.2294 & 0.3119 & 0.3761 \\ %& 0.4771 \\
\logmean (best HR@2)&  10 & 2 & 0.8  && 0.0734 & \textbf{0.1468} & 0.1927 & 0.2110 & 0.2477 & 0.3303 & 0.4037 \\ %& 0.4862 \\
\logmean (best HR@3)&  6  & 2 & 0.2  && 0.0642 & \textbf{0.1468} & \textbf{0.2110} & 0.2294 & \textbf{0.2569} & 0.3394 & 0.3945 \\ %& 0.5138
\logmean (best HR@4)&  6  & 2 & 0.0  && 0.0550 & 0.1376 & 0.1927 & \textbf{0.2477} & 0.2477 & \textbf{0.3486} & 0.3945 \\ % & 0.5046 \\
\logmean (best HR@5)&  4  & 1 & 0.8  && 0.0826 & \textbf{0.1468} & 0.1835 & 0.2018 & \textbf{0.2569} & 0.3394 & 0.4037 \\ %& 0.5138 \\
\logmean (best HR@10)& 10 & 2 & 0.0  && 0.0550 & 0.1376 & 0.1835 & 0.2294 & 0.2385 & \textbf{0.3486} & 0.3945 \\ %& 0.5046 \\
\logmean (best HR@20)& 4  & 1 & 1.0  && \textbf{0.0917} & 0.1376 & 0.1743 & 0.2294 & \textbf{0.2569} & 0.3211 & \textbf{0.4220} \\ %& 0.5046
\logmean 	    & all & 2 & 0.8  && 0.0734 & 0.1376 & 0.1835 & 0.2110 & 0.2477 & 0.3303 & 0.3945 \\
%log mean (best HR@40)& prev=3 alpha=0.1 & 0.0642 & 0.1376 & 0.1835 & 0.2202 & 0.2202 & \textbf{0.3486} & 0.3945 & \textbf{0.5229} \\

        \bottomrule
      \end{tabular}

 
  \end{threeparttable}


\vspace{15pt}


\small
  \caption{Performance Comparison for All Methods with Cut-off Time October 1st, 2014}
  \centering
  \label{tbl:results20141001}
  \begin{threeparttable}
     \vspace{-5pt}
      \begin{tabular}{
	@{\hspace{6pt}}l@{\hspace{6pt}}
        @{\hspace{0pt}}r@{\hspace{6pt}}
	@{\hspace{0pt}}r@{\hspace{6pt}}
        @{\hspace{0pt}}r@{\hspace{0pt}}
	@{\hspace{0pt}}l@{\hspace{6pt}}
	@{\hspace{0pt}}r@{\hspace{6pt}}          
	@{\hspace{6pt}}r@{\hspace{6pt}}
	@{\hspace{6pt}}r@{\hspace{6pt}}
	@{\hspace{6pt}}r@{\hspace{6pt}}
        @{\hspace{6pt}}r@{\hspace{6pt}}
        @{\hspace{6pt}}r@{\hspace{6pt}}
        @{\hspace{6pt}}r@{\hspace{6pt}}
        %@{\hspace{6pt}}r@{\hspace{6pt}}
	}
        \toprule
        method      & \multicolumn{3}{r}{parameters}  &  & HR@1  & HR@2 & HR@3 & HR@4 & HR@5 & HR@10 & HR@20 \\ %& HR@40 \\

        \midrule
\multirow{2}{*}{\baseline}  &   $s_p$ & $s_t$ & $\alpha$ & & \multirow{2}{*}{0.0750} & \multirow{2}{*}{0.1146} & \multirow{2}{*}{0.1479} & \multirow{2}{*}{0.1708} & \multirow{2}{*}{0.1979} & \multirow{2}{*}{0.2729} & \multirow{2}{*}{0.3479} \\ %& 0.4151 \\
\cline{2-4}
           &   $0.1$ & $0.1$ & $0.1$ & & & & & & & &\\
\personlized                 & & & & &              0.1500   & 0.1500 & 0.1500 & 0.1500 & 0.1500 & 0.1500 & 0.1500 \\   
\encounter                       & & & & &          0.1000   & 0.1500 & 0.1500 & 0.2000 & 0.2000 & 0.3000 & 0.4000 \\ 

\multirow{2}{*}{\HGN} & $n_h$ & $n_p$ & & &    \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{}  \\
\cline{2-3}
& $20$ & $3$  & && 0.0854 & 0.1250 & 0.1437 & 0.1604 & 0.1833 & 0.2354 & 0.3083\\

\multirow{2}{*}{\HAM} & $ n_h$ & $n_l$ & $n_p$ && \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{} & \multirow{2}{*}{}  \\   
\cline{2-4}
& $30$ & $3$  & $1$  && 0.0583 & 0.0854 & 0.1229 & 0.1521 & 0.1854 & 0.2396 & 0.3208 \\

        \midrule

        & $m_s$ & $m_c$  & $\alpha$ & & & & & & & &\\
\cline{2-4}
\logmean (best HR@1)& 10   & 1 & 0.0  && 0.1500 & 0.2000 & 0.2000 & 0.2500 & 0.2500 & 0.3500 & 0.4000 \\ 
\logmean (best HR@2)& 10   & 1 & 0.0  && 0.1500 & 0.2000 & 0.2000 & 0.2500 & 0.2500 & 0.3500 & 0.4000 \\
\logmean (best HR@3)& 10   & 1 & 0.0  && 0.1500 & 0.2000 & 0.2000 & 0.2500 & 0.2500 & 0.3500 & 0.4000 \\
\logmean (best HR@4)& 10   & 1 & 0.0  && 0.1500 & 0.2000 & 0.2000 & 0.2500 & 0.2500 & 0.3500 & 0.4000 \\
\logmean (best HR@5)& 10   & 1 & 0.0  && 0.1500 & 0.2000 & 0.2000 & 0.2500 & 0.2500 & 0.3500 & 0.4000 \\
\logmean (best HR@10)&10   & 1 & 0.0  && 0.1500 & 0.2000 & 0.2000 & 0.2500 & 0.2500 & 0.3500 & 0.4000 \\ 
\logmean (best HR@20)& 1   & 3 & 0.0  && 0.1000 & 0.1500 & 0.1500 & 0.2000 & 0.2000 & 0.3000 & 0.4500 \\
\logmean            & all & 1  & 0.0  && 0.1500 & 0.2000 & 0.2000 & 0.2500 & 0.2500 & 0.3500 & 0.4000 \\

        \bottomrule
      \end{tabular}

%      \begin{tablenotes}[normal,flushleft]
%      \begin{scriptsize}
%      \item
%          The best performance for each metric is \textbf{bold}.
%          The best performance among baseline methods is \underline{underlined}.
%          The best performance will not be marked if there is a large number 
%          of parameter settings that can get the same best performance.
          %
%          The parameter $n_h$ and $n_p$ for \HGN represent the number of training samples and 
%          the number of testing samples during training process, respectively. 
          %
%          The parameter $n_h$, $n_l$ and $n_p$ for \HAM represent the number of previous items in high-order 
%          associations, the number of previous items in low-order associations and the number of testing samples 
%          during training process, respectively.  
          %
%          The value ``all" for parameter $m_s$ indicating considering all previous search terms for recommendation.
%          \par
%      \end{scriptsize}
%      \end{tablenotes}


  \end{threeparttable}

\vspace{-5pt}
\end{table*}




\begin{table*}[!t]


\small
  \caption{Performance Comparison for All Methods with Cut-off Time April 1st, 2014}
  \centering
  \label{tbl:results20140401}
  \begin{threeparttable}
      \vspace{-5pt}
      \begin{tabular}{
	@{\hspace{6pt}}l@{\hspace{6pt}}
        @{\hspace{0pt}}r@{\hspace{6pt}}
	@{\hspace{0pt}}r@{\hspace{6pt}}
        @{\hspace{0pt}}r@{\hspace{0pt}}
	@{\hspace{0pt}}l@{\hspace{6pt}}
	@{\hspace{0pt}}r@{\hspace{6pt}}          
	@{\hspace{6pt}}r@{\hspace{6pt}}
	@{\hspace{6pt}}r@{\hspace{6pt}}
	@{\hspace{6pt}}r@{\hspace{6pt}}
        @{\hspace{6pt}}r@{\hspace{6pt}}
        @{\hspace{6pt}}r@{\hspace{6pt}}
        @{\hspace{6pt}}r@{\hspace{6pt}}
        %@{\hspace{6pt}}r@{\hspace{6pt}}
	}
        \toprule
        method      & \multicolumn{3}{r}{parameters}  &  & HR@1  & HR@2 & HR@3 & HR@4 & HR@5 & HR@10 & HR@20 \\ %& HR@40 \\

        \midrule
\multirow{2}{*}{\baseline}  &   $s_p$ & $s_t$ & $\alpha$ & & \multirow{2}{*}{0.1407} & \multirow{2}{*}{0.2024} & \multirow{2}{*}{0.2264} & \multirow{2}{*}{0.2436} & \multirow{2}{*}{0.2676} & \multirow{2}{*}{0.3276} & \multirow{2}{*}{0.3928} \\ 
\cline{2-4}
           &   $0.1$ & $0.1$ & $0.7$ & & & & & & & &\\
\personlized                 & & & & &              0.2302   & 0.2374 & 0.2734  & 0.2950  & 0.3094  & 0.3094  & 0.3094 \\   
\encounter                       & & & & &          \underline{0.3165}   & \underline{0.3453} & \underline{0.3741}  & \underline{0.3957}  & \underline{0.4029}  & \underline{0.4460}  & \underline{0.4820} \\ 

\multirow{2}{*}{\HGN} & $n_h$ & $n_p$ & & &    \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{}  \\
\cline{2-3}
& $2$  & $3$  & && 0.1458 & 0.1852 & 0.2075 & 0.2281 & 0.2556 & 0.2916 & 0.3688 \\

\multirow{2}{*}{\HAM} & $ n_h$ & $n_l$ & $n_p$ && \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{} & \multirow{2}{*}{}  \\   
\cline{2-4}
& $25$ & $3$  & $0$  && 0.0755 & 0.1578 & 0.2007 & 0.2367 & 0.2590 & 0.3002 & 0.3585 \\
        \midrule

        & $m_s$ & $m_c$  & $\alpha$ & & & & & & & &\\
\cline{2-4}
\logmean (best HR@1)&  10  & 1 & 0.2  && \textbf{0.3309} & 0.3525 & {0.4029} & 0.4101 & 0.4173 & 0.4532 & 0.5108 \\ 
\logmean (best HR@2)&  10  & 1 & 0.8  && 0.3094 & \textbf{0.3813} & {0.4029} & {0.4173} & 0.4173 & 0.4676 & {0.5324} \\
\logmean (best HR@3)&  7   & 1 & 0.4  && {0.3237} & {0.3597} & \textbf{0.4101} & \textbf{0.4245} & {0.4317} & 0.4460 & {0.5324} \\
\logmean (best HR@4)&  10  & 1 & 1.0  && 0.2806 & \textbf{0.3813} & {0.4029} & \textbf{0.4245} & {0.4317} & 0.4532 & 0.5180 \\
\logmean (best HR@5)&   5  & 3 & 0.8  && 0.3022 & {0.3597} & 0.3957 & {0.4173} & \textbf{0.4388} & {0.4748} & 0.5180 \\
\logmean (best HR@10)&  10 & 3 & 0.4  && {0.3237} & {0.3597} & 0.3885 & 0.4101 & 0.4245 & \textbf{0.4964} & 0.5180 \\
\logmean (best HR@20)&  2  & 1 & 0.8  && 0.2878 & 0.3381 & 0.3597 & 0.3597 & 0.3741 & 0.4388 & \textbf{0.5396} \\
\logmean            & all & 2  & 0.8  && 0.3094 & \textbf{0.3813} & {0.4029} & \textbf{0.4245} & {0.4317} & {0.4748} & 0.5252  \\

        \bottomrule
      \end{tabular}
  \end{threeparttable}



\vspace{15pt}

\small
  \caption{Performance Comparison for All Methods with Cut-off Time October 1st, 2013}
  \centering
  \label{tbl:results20131001}
  \begin{threeparttable}
    \vspace{-5pt} 
     \begin{tabular}{
	@{\hspace{6pt}}l@{\hspace{6pt}}
        @{\hspace{0pt}}r@{\hspace{6pt}}
	@{\hspace{0pt}}r@{\hspace{6pt}}
        @{\hspace{0pt}}r@{\hspace{0pt}}
	@{\hspace{0pt}}l@{\hspace{6pt}}
	@{\hspace{0pt}}r@{\hspace{6pt}}          
	@{\hspace{6pt}}r@{\hspace{6pt}}
	@{\hspace{6pt}}r@{\hspace{6pt}}
	@{\hspace{6pt}}r@{\hspace{6pt}}
        @{\hspace{6pt}}r@{\hspace{6pt}}
        @{\hspace{6pt}}r@{\hspace{6pt}}
        @{\hspace{6pt}}r@{\hspace{6pt}}
        %@{\hspace{6pt}}r@{\hspace{6pt}}
	}
        \toprule
        method      & \multicolumn{3}{r}{parameters}  &  & HR@1  & HR@2 & HR@3 & HR@4 & HR@5 & HR@10 & HR@20 \\ %& HR@40 \\

        \midrule
\multirow{2}{*}{\baseline}  &   $s_p$ & $s_t$ & $\alpha$ & & \multirow{2}{*}{0.0175} & \multirow{2}{*}{0.0234} & \multirow{2}{*}{0.0292} & \multirow{2}{*}{0.0351} & \multirow{2}{*}{0.0468} & \multirow{2}{*}{0.0760} & \multirow{2}{*}{0.1345} \\ %& 0.4151 \\
\cline{2-4}
           &   $0.1$ & $0.1$ & $0.7$ & & & & & & & &\\
\personlized                 & & & & &        0.1818   &  0.1818 & 0.1818 & 0.1818 & 0.1818 & 0.1818 & 0.1818\\   
\encounter                   & & & & &        0.0909   &  0.0909 & 0.0909 & 0.0909 & 0.2727 & 0.2727 & 0.2727 \\ 

\multirow{2}{*}{\HGN} & $n_h$ & $n_p$ & & &    \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{}  \\ 
\cline{2-3}
& $25$ & $3$  & && 0.0526 & 0.0643 & 0.0994 & 0.1053 & 0.1404 & 0.1637 & 0.2339 \\

\multirow{2}{*}{\HAM} & $ n_h$ & $n_l$ & $n_p$ && \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{} &  \multirow{2}{*}{} & \multirow{2}{*}{}  \\ 
\cline{2-4}
& $10$ & $3$  & $3$  && 0.0468 & 0.0994 & 0.1637 & 0.1696 & 0.1988 & 0.2456 & 0.3216 \\
        \midrule

	& $m_s$ & $m_c$  & $\alpha$ & & & & & & & &\\
\cline{2-4}
\logmean (best HR@1)&   10 & 1 & 0.0  && 0.0909 & 0.0909 & 0.1818 & 0.2727 & 0.2727 & 0.2727 & 0.2727 \\ 
\logmean (best HR@2)&   10 & 1 & 0.0  && 0.0909 & 0.0909 & 0.1818 & 0.2727 & 0.2727 & 0.2727 & 0.2727 \\
\logmean (best HR@3)&   10 & 1 & 0.0  && 0.0909 & 0.0909 & 0.1818 & 0.2727 & 0.2727 & 0.2727 & 0.2727 \\
\logmean (best HR@4)&   10 & 1 & 0.0  && 0.0909 & 0.0909 & 0.1818 & 0.2727 & 0.2727 & 0.2727 & 0.2727 \\
\logmean (best HR@5)&   10 & 1 & 0.0  && 0.0909 & 0.0909 & 0.1818 & 0.2727 & 0.2727 & 0.2727 & 0.2727 \\
\logmean (best HR@10)&  10 & 3 & 0.0  && 0.0909 & 0.0909 & 0.0909 & 0.0909 & 0.2727 & 0.3636 & 0.3636 \\
\logmean (best HR@20)&  1  & 3 & 0.2  && 0.0909 & 0.0909 & 0.0909 & 0.0909 & 0.1818 & 0.1818 & 0.4545 \\
\logmean            & all & 1  & 0.0  && 0.0909 & 0.0909 & 0.1818 & 0.2727 & 0.2727 & 0.2727 & 0.2727 \\

        \bottomrule
      \end{tabular}

      \begin{tablenotes}[normal,flushleft]
      \begin{scriptsize}
      \item
         For Table \ref{tbl:results20150401}, \ref{tbl:results20141001}, \ref{tbl:results20140401} and 
         \ref{tbl:results20131001}, 
          the best performance for each metric is \textbf{bold}.
          The best performance among baseline methods is \underline{underlined}.
          The best performance will not be marked if there is a large number 
          of parameter settings that can get the same best performance.
          %
          The parameter $n_h$ and $n_p$ for \HGN represent the number of training samples and
          the number of testing samples during training process, respectively.
          %
          The parameter $n_h$, $n_l$ and $n_p$ for \HAM represent the number of previous items in high-order
          associations, the number of previous items in low-order associations and the number of testing samples 
          during training process, respectively. 
          %
          The value ``all" for parameter $m_s$ indicating considering all previous search terms for recommendation. 
         \par
      \end{scriptsize}
      \end{tablenotes}
 
  \end{threeparttable}

\end{table*}





==> tables/statistics_combine.tex <==
\begin{table}[t]

\begin{minipage}[t]{0.4\textwidth}
\small
  \caption{Dataset Statistics}
  \centering
  \vspace{-8pt}
  \label{tbl:dataset}
  \begin{threeparttable}
     \begin{footnotesize}
      \begin{tabular}{
        @{\hspace{0pt}}l@{\hspace{8pt}}
        @{\hspace{8pt}}r@{\hspace{8pt}}
        }
        \toprule
        \# of patients & 2,955 \\
        \# of search terms & 2,540 \\
        \# of ICD 9 codes & 7,027 \\
        \# of encounters & 511,987 \\
        \# of search term sessions & 3,488 \\
        \midrule
        Avg. \# of search terms per patient & 10.22 \\
        Avg. \# of encounters per patient & 173.26 \\
        Avg. \# of ICD 9 codes per encounter & 2.09 \\
        Avg. \# of searches per term & 24 \\
        Avg. \# of previous encounters per term & 228.89 \\ 
        Avg. \# of search term sessions per patient & 1.18 \\
        Avg. \# of search terms per session & 8.66 \\
        \bottomrule
      \end{tabular}
      \end{footnotesize}

    %  \begin{tablenotes}[normal,flushleft]
    %  \begin{scriptsize}

    %  \end{scriptsize}
    %  \end{tablenotes}
  \end{threeparttable}
\end{minipage}
%
%
\begin{minipage}[t]{0.25\textwidth}
    \centering
    \vspace{0pt}
    \raisebox{-\height}{\includegraphics[width=\linewidth]{patient_session_hist.pdf}}
    \captionof{figure}{Histogram of Paitents in terms of Number of Search Terms Sessions}
        \label{fig:patient_session_hist}
\end{minipage}%
%
%
\begin{minipage}[t]{0.3\textwidth}
    \centering
    \vspace{0pt}
    \raisebox{-\height}{\includegraphics[width=\linewidth]{session_term_hist.pdf}}
    \captionof{figure}{Histogram of Sessions in terms of Number of Search Terms per Session}
        \label{fig:session_term_hist}
\end{minipage}%
\end{table}



